Counterfactual Inference for Consumer Choice Across Many Product Categories

This paper proposes a method for estimating consumer preferences among discrete choices, where the consumer chooses at most one product in a category, but selects from multiple categories in parallel. The consumer's utility is additive in the different categories. Her preferences about product attributes as well as her price sensitivity vary across products and are in general correlated across products. We build on techniques from the machine learning literature on probabilistic models of matrix factorization, extending the methods to account for time-varying product attributes and products going out of stock. We evaluate the performance of the model using held-out data from weeks with price changes or out of stock products. We show that our model improves over traditional modeling approaches that consider each category in isolation. One source of the improvement is the ability of the model to accurately estimate heterogeneity in preferences (by pooling information across categories); another source of improvement is its ability to estimate the preferences of consumers who have rarely or never made a purchase in a given category in the training data. Using held-out data, we show that our model can accurately distinguish which consumers are most price sensitive to a given product. We consider counterfactuals such as personally targeted price discounts, showing that using a richer model such as the one we propose substantially increases the benefits of personalization in discounts.

==> CounterfactualFit.tex <==
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Individual} & \multicolumn{2}{c}{Aggregate} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5}
Model & Popular & Less Common & Popular & Less Common\\
\midrule
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{All Weeks}}\\
\hspace{1em}Nested Factorization & -0.1070 (0.0004) & -0.0173 (0.0001) & -2.5356 (0.0146) & -1.3072 (0.0044)\\
\hspace{1em}Mixed Logit with Random Price and HPF Controls & -0.1156 (0.0004) & -0.0188 (0.0001) & -2.5562 (0.0145) & -1.3365 (0.0037)\\
\hspace{1em}Nested Logit with HPF Controls & -0.1194 (0.0005) & -0.0191 (0.0001) & -2.5568 (0.0154) & -1.3105 (0.0040)\\
\hspace{1em}Multinomial Logit with HPF Controls & -0.1194 (0.0005) & -0.0191 (0.0001) & -2.5554 (0.0154) & -1.3086 (0.0040)\\
\hspace{1em}Mixed Logit with Random Price and Random Intercepts & -0.1263 (0.0005) & -0.0194 (0.0001) & -2.5712 (0.0146) & -1.3316 (0.0037)\\
\hspace{1em}Mixed Logit with Random Price and Demographics & -0.1240 (0.0004) & -0.0195 (0.0001) & -2.5934 (0.0153) & -1.3543 (0.0038)\\
\hspace{1em}Multinomial Logit with Demographic Controls & -0.1290 (0.0005) & -0.0197 (0.0001) & -2.5722 (0.0157) & -1.3105 (0.0040)\\
\hspace{1em}Nested Logit with Demographic Controls & -0.1289 (0.0005) & -0.0197 (0.0001) & -2.5740 (0.0157) & -1.3113 (0.0041)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{Cross Price Weeks}}\\
\hspace{1em}Nested Factorization & -0.0925 (0.0008) & -0.0149 (0.0001) & -2.4527 (0.0262) & -1.2017 (0.0084)\\
\hspace{1em}Mixed Logit with Random Price and HPF Controls & -0.1006 (0.0008) & -0.0163 (0.0001) & -2.4846 (0.0258) & -1.2584 (0.0069)\\
\hspace{1em}Nested Logit with HPF Controls & -0.1041 (0.0009) & -0.0164 (0.0001) & -2.4844 (0.0277) & -1.2177 (0.0076)\\
\hspace{1em}Multinomial Logit with HPF Controls & -0.1041 (0.0009) & -0.0164 (0.0001) & -2.4836 (0.0276) & -1.2165 (0.0076)\\
\hspace{1em}Mixed Logit with Random Price and Random Intercepts & -0.1139 (0.0009) & -0.0168 (0.0001) & -2.5002 (0.0260) & -1.2527 (0.0069)\\
\hspace{1em}Mixed Logit with Random Price and Demographics & -0.1111 (0.0009) & -0.0170 (0.0001) & -2.5132 (0.0280) & -1.2752 (0.0071)\\
\hspace{1em}Multinomial Logit with Demographic Controls & -0.1162 (0.0010) & -0.0170 (0.0001) & -2.4966 (0.0279) & -1.2182 (0.0077)\\
\hspace{1em}Nested Logit with Demographic Controls & -0.1161 (0.0010) & -0.0170 (0.0001) & -2.5066 (0.0292) & -1.2194 (0.0078)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{Own Price Weeks}}\\
\hspace{1em}Nested Factorization & -0.1374 (0.0009) & -0.0229 (0.0001) & -2.7871 (0.0360) & -1.5544 (0.0104)\\
\hspace{1em}Mixed Logit with Random Price and HPF Controls & -0.1465 (0.0009) & -0.0243 (0.0001) & -2.8004 (0.0357) & -1.5475 (0.0086)\\
\hspace{1em}Nested Logit with HPF Controls & -0.1493 (0.0009) & -0.0249 (0.0001) & -2.7986 (0.0371) & -1.5356 (0.0092)\\
\hspace{1em}Multinomial Logit with HPF Controls & -0.1493 (0.0009) & -0.0249 (0.0001) & -2.7949 (0.0373) & -1.5321 (0.0092)\\
\hspace{1em}Mixed Logit with Random Price and Random Intercepts & -0.1530 (0.0009) & -0.0251 (0.0001) & -2.8003 (0.0348) & -1.5408 (0.0085)\\
\hspace{1em}Mixed Logit with Random Price and Demographics & -0.1525 (0.0009) & -0.0251 (0.0001) & -2.8544 (0.0374) & -1.5709 (0.0090)\\
\hspace{1em}Multinomial Logit with Demographic Controls & -0.1557 (0.0010) & -0.0256 (0.0002) & -2.8097 (0.0369) & -1.5344 (0.0092)\\
\hspace{1em}Nested Logit with Demographic Controls & -0.1555 (0.0010) & -0.0256 (0.0002) & -2.8186 (0.0372) & -1.5377 (0.0093)\\
\addlinespace[0.3em]
\multicolumn{5}{l}{\textbf{Out of Stock Weeks}}\\
\hspace{1em}Nested Factorization & -0.0924 (0.0040) & -0.0159 (0.0002) & -2.3349 (0.1114) & -1.2746 (0.0129)\\
\hspace{1em}Mixed Logit with Random Price and HPF Controls & -0.1033 (0.0044) & -0.0173 (0.0002) & -2.3679 (0.1225) & -1.3064 (0.0111)\\
\hspace{1em}Nested Logit with HPF Controls & -0.1068 (0.0046) & -0.0176 (0.0002) & -2.3427 (0.1243) & -1.2817 (0.0122)\\
\hspace{1em}Multinomial Logit with HPF Controls & -0.1068 (0.0046) & -0.0176 (0.0002) & -2.3446 (0.1259) & -1.2774 (0.0121)\\
\hspace{1em}Mixed Logit with Random Price and Demographics & -0.1091 (0.0045) & -0.0180 (0.0002) & -2.3669 (0.1132) & -1.3249 (0.0118)\\
\hspace{1em}Mixed Logit with Random Price and Random Intercepts & -0.1125 (0.0046) & -0.0181 (0.0002) & -2.3403 (0.1156) & -1.3068 (0.0113)\\
\hspace{1em}Multinomial Logit with Demographic Controls & -0.1146 (0.0048) & -0.0183 (0.0002) & -2.3261 (0.1189) & -1.2800 (0.0122)\\
\hspace{1em}Nested Logit with Demographic Controls & -0.1145 (0.0047) & -0.0183 (0.0002) & -2.2974 (0.0990) & -1.2840 (0.0123)\\
\bottomrule
\end{tabular}}


==> Elasticities.tex <==
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Own Price} & \multicolumn{3}{c}{Class Cross Price} & \multicolumn{3}{c}{Subclass Cross Price} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7} \cmidrule(l{3pt}r{3pt}){8-10}
Model & Median & SD(Mean) & Mean(SD) & Inside & Outside & \% & Inside & Outside & \%\\
\midrule
Nested Factorization & -1.7121 & 1.2008 & 1.7774 & 0.0186 & 0.0080 & 132\% & 0.0196 & 0.0181 & 8.4\%\\
Nested Logit with Demographic Controls & -1.2976 & 1.0377 & 0.0532 & 0.0119 & 0.0086 & 37\% & 0.0125 & 0.0115 & 8.5\%\\
Mixed Logit with Random Price and Random Intercepts & -2.2024 & 1.7822 & 0.8387 & 0.0062 & 0.0053 & 16\% & 0.0062 & 0.0062 & -0.7\%\\
Mixed Logit with Random Price and HPF Controls & -2.7077 & 1.9084 & 1.1294 & 0.0063 & 0.0054 & 16\% & 0.0063 & 0.0065 & -3.9\%\\
Multinomial Logit with HPF Controls & -1.1841 & 0.8904 & 0.0060 & 0.0035 & 0.0030 & 16\% & 0.0036 & 0.0035 & 0.8\%\\
\addlinespace
Multinomial Logit with Demographic Controls & -1.1813 & 0.8837 & 0.0017 & 0.0034 & 0.0029 & 16\% & 0.0034 & 0.0034 & 2.1\%\\
Mixed Logit with Random Price and Demographics & -3.0897 & 2.4546 & 1.4785 & 0.0067 & 0.0060 & 13\% & 0.0066 & 0.0069 & -4.6\%\\
Nested Logit with HPF Controls & -1.1017 & 0.8783 & 0.0182 & 0.0148 & 0.0158 & -7\% & 0.0140 & 0.0157 & -10.7\%\\
\bottomrule
\end{tabular}}


==> Elasticities_cross.tex <==
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{1}{c}{ } &  \multicolumn{3}{c}{Class Cross Price} & \multicolumn{3}{c}{Subclass Cross Price} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
Model                                               & Inside & Outside & \%    & Inside & Outside & \%\\
\midrule
Nested Factorization                                & 0.0186 & 0.0080  & 132\% & 0.0196 & 0.0181  & 8.4\%\\
Nested Logit with Demographic Controls              & 0.0119 & 0.0086  & 37\%  & 0.0125 & 0.0115  & 8.5\%\\
Mixed Logit with Random Price and Random Intercepts & 0.0062 & 0.0053  & 16\%  & 0.0062 & 0.0062  & -0.7\%\\
Mixed Logit with Random Price and HPF Controls      & 0.0063 & 0.0054  & 16\%  & 0.0063 & 0.0065  & -3.9\%\\
Multinomial Logit with HPF Controls                 & 0.0035 & 0.0030  & 16\%  & 0.0036 & 0.0035  & 0.8\%\\
Multinomial Logit with Demographic Controls         & 0.0034 & 0.0029  & 16\%  & 0.0034 & 0.0034  & 2.1\%\\
Mixed Logit with Random Price and Demographics      & 0.0067 & 0.0060  & 13\%  & 0.0066 & 0.0069  & -4.6\%\\
Nested Logit with HPF Controls                      & 0.0148 & 0.0158  & -7\%  & 0.0140 & 0.0157  & -10.7\%\\
\bottomrule
\end{tabular}}

==> Elasticities_own.tex <==
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Own Price} \\
\cmidrule(l{3pt}r{3pt}){2-4}
Model                                               & Median  & SD(Mean) & Mean(SD) \\
\midrule
Nested Factorization                                & -1.7121 & 1.2008   & 1.7774 \\
Nested Logit with Demographic Controls              & -1.2976 & 1.0377   & 0.0532 \\
Mixed Logit with Random Price and Random Intercepts & -2.2024 & 1.7822   & 0.8387 \\
Mixed Logit with Random Price and HPF Controls      & -2.7077 & 1.9084   & 1.1294 \\
Multinomial Logit with HPF Controls                 & -1.1841 & 0.8904   & 0.0060 \\
Multinomial Logit with Demographic Controls         & -1.1813 & 0.8837   & 0.0017 \\
Mixed Logit with Random Price and Demographics      & -3.0897 & 2.4546   & 1.4785 \\
Nested Logit with HPF Controls                      & -1.1017 & 0.8783   & 0.0182 \\
\bottomrule
\end{tabular}}


==> FitByCategory.tex <==
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Mean Rank} & \multicolumn{2}{c}{\% Best Performance} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5}
Model & Log L & SE & Log L & SE\\
\midrule
Nested Factorization & 1.53 & 1.10 & 86.2\% & 95.9\%\\
Mixed Logit with Random Price and HPF Controls & 2.40 & 5.33 & 9.8\% & 0.8\%\\
Nested Logit with HPF Controls & 3.87 & 3.38 & 0.0\% & 0.8\%\\
Multinomial Logit with HPF Controls & 4.21 & 3.63 & 0.8\% & 0.8\%\\
Mixed Logit with Random Price and Random Intercepts & 4.69 & 5.65 & 0.8\% & 1.6\%\\
\addlinespace
Mixed Logit with Random Price and Demographics & 5.21 & 7.07 & 2.4\% & 0.0\%\\
Nested Logit with Demographic Controls & 6.96 & 4.93 & 0.0\% & 0.0\%\\
Multinomial Logit with Demographic Controls & 7.13 & 4.91 & 0.0\% & 0.0\%\\
\bottomrule
\end{tabular}}


==> Personalization.tex <==
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Coef of Variation} & \multicolumn{2}{c}{Regression Coef} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5}
Model & UPC & Category & UPC & Category\\
\midrule
Nested Factorization & 3.2546 & 1.7756 & 0.9955 & 1.0023\\
Mixed Logit with Random Price and HPF Controls & 2.0747 & 1.6085 & 0.6861 & 0.7007\\
Mixed Logit with Random Price and Demographics & 1.3869 & 1.5724 & 0.4718 & 0.5968\\
Multinomial Logit with HPF Controls & 1.2590 & 0.7276 & 0.8402 & 0.8893\\
Nested Logit with HPF Controls & 1.2368 & 0.7520 & 0.8417 & 0.8725\\
\addlinespace
Mixed Logit with Random Price and Random Intercepts & 1.0834 & 1.0446 & 0.4666 & 0.6959\\
Nested Logit with Demographic Controls & 0.4465 & 0.2967 & 0.8947 & 0.9314\\
Multinomial Logit with Demographic Controls & 0.4337 & 0.2756 & 0.9077 & 0.9411\\
\bottomrule
\end{tabular}}


==> PredictiveFit.tex <==
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Mean Log Likelihood} & \multicolumn{2}{c}{Mean Squared Error} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5}
Model & Train & Test & Train & Test\\
\midrule
Nested Factorization & -4.2271 & -4.9096 & 0.8981 & 0.9268\\
Mixed Logit with Random Price and HPF Controls & -4.9233 & -5.3125 & 0.9473 & 0.9660\\
Nested Logit with HPF Controls & -5.2345 & -5.4230 & 0.9583 & 0.9650\\
Multinomial Logit with HPF Controls & -5.2307 & -5.4248 & 0.9583 & 0.9651\\
Mixed Logit with Random Price and Demographics & -5.2976 & -5.5690 & 0.9780 & 0.9898\\
\addlinespace
Mixed Logit with Random Price and Random Intercepts & -5.3956 & -5.5827 & 0.9785 & 0.9849\\
Nested Logit with Demographic Controls & -5.6080 & -5.6779 & 0.9788 & 0.9801\\
Multinomial Logit with Demographic Controls & -5.6142 & -5.6791 & 0.9791 & 0.9803\\
\bottomrule
\end{tabular}}


==> couponTargeting.tex <==
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{\% Gains Relative to Uniform} \\
\cmidrule(l{3pt}r{3pt}){2-4}
Model & Behavioral & Demographic & Individualized\\
\midrule
Nested Factorization (linear) & 2.57\% & 4.55\% & 28.5\%\\
Mixed Logit with Random Price Effects and HPF Controls (linear) & 1.51\% & 2.38\% & 5.7\%\\
Multinomial Logit with HPF Controls (linear) & 1.37\% & 1.60\% & 5.7\%\\
Nested Logit with HPF Controls (linear) & 1.41\% & 1.57\% & 5.4\%\\
Nested Logit with Demographic Controls (linear) & 0.56\% & 3.03\% & 4.7\%\\
\addlinespace
Multinomial Logit with Demographic Controls (linear) & 0.77\% & 2.17\% & 3.4\%\\
Mixed Logit with Random Price Effects and Demographics (linear) & 0.75\% & 2.53\% & 3.1\%\\
Mixed Logit with Random Price and Random Intercepts (linear) & 0.86\% & 1.31\% & 2.5\%\\
\bottomrule
\end{tabular}}

